Affordance Perception by a Knowledge-Guided Vision-Language Model with Efficient Error Correction

Mobile robot platforms will increasingly be tasked with activities that involve grasping and manipulating objects in open world environments. Affordance understanding provides a robot with means to realise its goals and execute its tasks, e.g. to achieve autonomous navigation in unknown buildings where it has to find doors and ways to open these. In order to get actionable suggestions, robots need to be able to distinguish subtle differences between objects, as they may result in different action sequences: doorknobs require grasp and twist, while handlebars require grasp and push. In this paper, we improve affordance perception for a robot in an open-world setting. Our contribution is threefold: (1) We provide an affordance representation with precise, actionable affordances; (2) We connect this knowledge base to a foundational vision-language models (VLM) and prompt the VLM for a wider variety of new and unseen objects; (3) We apply a human-in-the-loop for corrections on the output of the VLM. The mix of affordance representation, image detection and a human-in-the-loop is effective for a robot to search for objects to achieve its goals. We have demonstrated this in a scenario of finding various doors and the many different ways to open them.

==> sections/contribution.tex <==
\section{Contribution :: dit moet in een strakke vorm naar de Introduction verhuizen}

Leveraging foundational vision-language models with HitL to perceive actionable affordances



\hl{GertJan}
Ik denk aan: (A) Voor perceptie van affordances moet er kennis zijn over de objecten, waarvoor ze gebruikt kunnen worden, en hoe ze ingezet kunnen worden. Zo'n model kan uit een knowledge-base of LLM komen, maar vergt wat shaping om het actionable te maken. Op dit moment moet dat nog handmatig. Schaaphok, M.W. (Marianne), kunnen we dit staven met ChatGPT, dat dit inderdaad niet as-is bruikbaar is? Een voorbeeld zou wel sterk zijn als onderbouwing. Daarom stellen we een model voor met relaties voor in de vorm van X-Y-Z -> Schaaphok, M.W. (Marianne) jouw invulling hier. (B) Voor perceptie van de relevante objecten, is het belangrijk om zonder veel inspanning / voorbereidingstijd om te kunnen gaan met nieuwe kennis uit punt A. Daarom kijken we naar vision-language modellen zoals GLIP die promptable zijn voor nieuwe of andere objecten. Interessante bevinding dat ze niet goed onderscheid kunnen maken in details die er voor actions juist erg toe doen -> voorbeeld handle/knob. Dat is op het eerste oog verrassend, want ChatGPT weet het verschil erg goed -> snippets van Marianne laten zien. Maar blijkbaar kunnen een VLM zoals GLIP dit niet onderscheiden -> dit is een inzicht/bijdrage op zichzelf. (C) Daarom stellen we een human-in-the-loop voor, waarbij een robot een eerste ronde doet, daarna een tussenstap om uit de gevonden objecten er snel een paar te hernoemen, leidend tot een beter model dat meer actionable is -> snapshots uit filmpje, link naar filmpje, en performance grafiek.



\hl{Marianne} 
\begin{itemize}
    \item manier van affordance weergave die het mogelijk maakt om actionable hiermee om te gaan en op basis hiervan te kunnen redeneren over welke impact met welke objecten gehaald kan worden en welke actie daarvoor nodig is.
    \item voor actionable suggesties over welke actie een robot moet doen kunnen nuances belangrijk zijn, hiervoor zijn huidge LVM niet altijd goed genoeg. 
    \item met een human-in-the-loop kunnen dit soort nuance verschillen snel worden gecorrigeerd dmv clustering en annotaties. 
\end{itemize}  



